How BlockChain Can Help Enhance The Security And Privacy in Edge Computing?

In order to solve security and privacy issues of centralized cloud services, the edge computing network is introduced, where computing and storage resources are distributed to the edge of the network. However, native edge computing is subject to the limited performance of edge devices, which causes challenges in data authorization, data encryption, user privacy, and other fields. Blockchain is currently the hottest technology for distributed networks. It solves the consistent issue of distributed data and is used in many areas, such as cryptocurrency, smart grid, and the Internet of Things. Our work discussed the security and privacy challenges of edge computing networks. From the perspectives of data authorization, encryption, and user privacy, we analyze the solutions brought by blockchain technology to edge computing networks. In this work, we deeply present the benefits from the integration of the edge computing network and blockchain technology, which effectively controls the data authorization and data encryption of the edge network and enhances the architecture's scalability under the premise of ensuring security and privacy. Finally, we investigate challenges on storage, workload, and latency for future research in this field.

==> images/mainflow.tex <==
% \section{Diagrammatic view of Multisketch operations}\label{app:mainflow}  

% A user registers with a user id $\u$ and a vector of biometric templates
% $\mvec=\mvecss{\mlen}$. Multisketch uses two databases $\dbid$ and $\dbmsg$\@,
% where $\dbid$ contains user id $\u$ and the corresponding helper data
% $\sketchval$, and $\dbmsg$ contains the random permutation of the templates
% registered so far. Highlighted are the entries corresponding to a user $\u_4$
% with templates $\mvec_4=\mvec_{41}\ldots\mvec_{4\mlen}$.% and helper
%     % data $\sketchval_4$.
\begin{figure}[t]
  \centering
  \begin{tikzpicture}[
    >=stealth,
    node distance=2cm,
    database/.style={
      cylinder,
      cylinder uses custom fill,
      cylinder body fill=black!25!white,
      cylinder end fill=black!25!white,
      shape border rotate=90,
      aspect=0.25,
      minimum width=2em,
      minimum height=2em,
      draw
    },
    func/.style={
      rectangle,
      fill=red!25!white,
      minimum width=1cm,
      minimum height=1em,
      draw
    },
    cell/.style={
      rectangle,
      draw=black!50!white
    }
    ]
    \node (user) at (0, 0) {User};
    \node[func, right of=user, right=-1.1em, above=3em] (msketch) {$\MS$}; 
    \draw[below of=msketch, dashed, anchor=west] (.85,0.55) rectangle (5.9,-1.2); 
    \node[func, below of=msketch, anchor=east, below=1.95cm,fill=red!10!white,dashed] (mrecover) {$\MRec$};
    % \node[database, right of=user, anchor=south, above=1em, right=2cm] (db1) {$\dbid$};
    \matrix (db1) [right of=user, anchor=south, below=2pt, right=-0.1cm, 
    matrix of math nodes,
    column sep = -\pgflinewidth,
    row sep=-\pgflinewidth,
    column 1/.style={nodes={cell}}, 
    column 2/.style={nodes={cell}}, 
    anchor=west] {
      \u_1 & \sketchval_1\\
      \u_2 & \sketchval_2\\
      \u_3 & \sketchval_3\\
      |[draw,fill=blue!20]|\u_4 & |[draw,fill=blue!20]|\sketchval_4\\
    };
    \node[left of=db1, anchor=east,right=1.1cm] {$\dbid$};
    \matrix (db2) [right of=db1, left=25pt, matrix of math nodes,
    column sep = 2\pgflinewidth,
    row sep=-\pgflinewidth,
    column 1/.style={nodes={cell}},
    column 2/.style={nodes={cell}}, 
    column 3/.style={nodes={cell}}, 
    column 4/.style={nodes={cell}}, 
    column 5/.style={nodes={cell}}, 
    anchor=west] {
      \mvec_{21} &\mvec_{12} & |[draw,fill=blue!20]|\mvec_{43} &  & \mvec_{3\mlen} \\
      |[draw,fill=blue!20]|\mvec_{41} &\mvec_{32} & \mvec_{33} & |[draw=white]|\ldots & \mvec_{2\mlen} \\
      \mvec_{11} &|[draw,fill=blue!20]|\mvec_{42} & \mvec_{23} &  & \mvec_{1\mlen} \\
      \mvec_{31} &\mvec_{22} & \mvec_{13} & & |[draw,fill=blue!20]|\mvec_{4\mlen} \\
    };
    \node[left of=db2, left=-4pt] {$\dbmsg$};

    % \node[database,right of=db1] (db2) {$\dbmsg$};
    \node[func,below of=db1,anchor=north,above=8pt,left=8pt] (gu) {GetUser};
    \node[func,right of=gu,anchor=east,right=-5pt] (fm) {FindMatches};
    \node[func,below of=db1,anchor=east,below=2em,right=-3pt] (recover) {Recover};

    \draw[->,blue!50,thick] (user.north) |- node[black,near end,above]{$u, \mvec$} node[black,near end,below,font=\small]{register} 
    (msketch.west);
    \draw[->,blue!50,thick] (msketch) -| node[black,near end, left,right]{$u, \sketchval$} (db1);
    \draw[->,blue!50,thick] (msketch) -| node[black,near end, left,right]{$\mvec$} (db2);

    \draw[->,blue!50,thick] (user.south) |- ++(1,-0.9) node[black,near end,above]{$u, \mvectilde$} node[black,near end,below,font=\small]{login}   -| node[black,left,near end]{$u$}
    (gu.north);
    \draw[->,blue!50,thick] (user.south) |- ++(0,-0.9)  -- ++(3.1,0) |- node[black,near end, above]{$\mvectilde$}
    (fm.west);
    \draw[->,blue!50,thick] (db1.south) |- node[black,near end,above]{} (gu.east);
    \draw[->,blue!50,thick] (db2.south) |- node[black,near end,above]{} (fm.east);
    \draw[->,blue!50,thick] (gu.south) |- node[black,near end,above]{$\sketchval$} (recover.west);
    \draw[->,blue!50,thick] (fm.south) |- node[black,near end,above]{$\mvec'$} (recover.east);    
    \draw[->,blue!50,line width=2pt] (recover.south) -- node[black,near end,right]{$\mvec$ or $\bot$} ++(0, -0.65);
  \end{tikzpicture}
  % \rcnote{Rough sketch of the flow of the \biosketch.} 
  \caption{Diagram of multisketch as a part of an authentication service. 
  }
  \label{fig:mainflow}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

